HyTasker: Hybrid Task Allocation in Mobile Crowd Sensing

Task allocation is a major challenge in Mobile Crowd Sensing (MCS). While previous task allocation approaches follow either the opportunistic or participatory mode, this paper proposes to integrate these two complementary modes in a two-phased hybrid framework called HyTasker. In the offline phase, a group of workers (called opportunistic workers) are selected, and they complete MCS tasks during their daily routines (i.e., opportunistic mode). In the online phase, we assign another set of workers (called participatory workers) and require them to move specifically to perform tasks that are not completed by the opportunistic workers (i.e., participatory mode). Instead of considering these two phases separately, HyTasker jointly optimizes them with a total incentive budget constraint. In particular, when selecting opportunistic workers in the offline phase of HyTasker, we propose a novel algorithm that simultaneously considers the predicted task assignment for the participatory workers, in which the density and mobility of participatory workers are taken into account. Experiments on a real-world mobility dataset demonstrate that HyTasker outperforms other methods with more completed tasks under the same budget constraint.

==> oppo.tex <==
\section{OPPORTUNISTIC WORKER SELECTION}

\subsection{Main Process and Basic Idea}
As mentioned in previous sections, the key technical challenge of HyTasker lies in how to do the offline opportunistic worker selection, in which the future possible task assignment of the participatory workers should be jointly considered. To address this challenge, we propose a nested-loop process (see Algorithm ~\ref{alg:OWS}).The inner-loop searches and determines which opportunistic worker should be selected, while the outer-loop process estimates the number of completed tasks for a given subset of opportunistic workers and predicted task assignment of the participatory workers. Finally, the output is the subset of the opportunistic workers that achieves the maximum estimated number of completed tasks. 

\algrenewcommand{\algorithmiccomment}[1]{\hfill$\blacktriangleright$ #1}
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}
\begin{algorithm}[htb]         %算法的开始
	\caption{Opportunistic Worker Selection Algorithm}             %算法的标题
	\label{alg:OWS}                  %给算法一个标签，这样方便在文中对算法的引用
	\begin{algorithmic}[1]                %不知[1]是干嘛的？
		\Require candidate opportunistic workers $OW$; candidate participatory workers $PW$; total budget constraint $B$.
		\Ensure the best candidate opportunistic workers $OW_f$.
		
		\State set $OW_f=OW_f^{'}=\varnothing$
		\State set $TW_f=0$
		\While {$|OW_f^{'}|*I_c<B$}
			\State set $MaxUtility=0$
			\For{each $ow_j\in OW/OW_f^{'}$}
			 \If{$Utility(OW_f^{'}\cup \{ow_j\})>MaxUtility$}
		     \State $MaxUtility=Utility(OW_f^{'}\cup \{ow_j\})$ \Comment{$Utility(OW_f)$ will be defined in section 4.2.2}
		     \State $BestW=ow_j$
		 	 \EndIf
			\EndFor
			
			\State $OW_f^{'} = OW_f^{'} \cup \{ow_j\}$
			\State $OW=OW-\{ow_j\}$
			\State $PredicateOnlineAssign(PW,B-I_c*|OW_f^{'}|)$
			
			\If{$TW>TW_f$} \Comment{$TW$ will be described in detail in section 4.2.3}
			\State $OW_f=OW_f^{'}$
			\EndIf
			%\STATE select $w_u$ from $OW/OW_f^{'}$ with maximum $Utility(OW_f^{'}\cup \{w_u\})$ \\
			
			
			%\STATE $flag=networkSpread(U^{'}, q)$
		\EndWhile	
		
		\Return $OW_f$ 
	\end{algorithmic}
\end{algorithm}


The above process is more technically challenging and complicated than the state-of-the-art studies for opportunistic worker selection such as [16,19,22,21] in the following two aspects.


First, for the inner loop, the challenge is how to select the most beneficial opportunistic workers. Existing studies incrementally select workers with the highest estimated coverage gain [16,19,22,21]. However, HyTasker should further consider the future online task assignment of the participatory workers. Specifically, this inner-loop process is designed based on a key idea, that is, we prefer to select the opportunistic workers with two characteristics: (1) those workers who can complete more tasks; 2) those workers who can complete tasks located in areas where the participatory workers are sparsely distributed according to the historical mobility records. As Fig. ~\ref{fig_2} shows, we assign higher priority to the opportunistic worker A than B, because A is more likely to complete tasks within areas where the participatory workers are sparsely distributed. In this paper, we introduce the concept of location entropy [31] in social network community to realize this idea, which will be described in section 4.2.2 with more details.


Second, for the existing work [16,19,22,21], the worker selection process ends when the total budget has been used up, and the finally obtained set of workers is the output. However, in our problem, it is not optimal if we spend all the budget on the opportunistic workers. Therefore, after adding and selecting one worker, we record the obtained subset of opportunistic workers as a snapshot. Ultimately, we determine which subset (snapshot) should be selected by simultaneously considering the predicted task assignments of the participatory workers online (line 13\texttildelow 16 in Algorithm~\ref{alg:OWS}). This component will be illustrated with more details in section 4.2.3.

\begin{figure}[!t]
	
	\centering \includegraphics[width=.4\textwidth]{pic/fig2.png}
	
	\caption{An example to illustrate the priority of opportunistic workers (we assign higher priority to worker A than B, because A is more likely to complete tasks in areas where the participatory workers are sparsely distributed)  \label{fig_2}}
\end{figure}


\subsection{Core Supporting Algorithms}

To implement the algorithm ~\ref{alg:OWS}, we need to further design three supporting algorithms. First, we need to predict the mobility of all candidate workers (section 4.2.1). Second, for the inner loop, we should determine which worker should be selected (section 4.2.2). Third, as the execution of each iteration forms a feasible solution (one snapshot), we should further determine which one is the optimal (section 4.2.3). 

\subsubsection{Mobility prediction}
Similar to [19,22,23], this paper assumes that the sensing range of a task is within a cell tower's connection, and the opportunistic workers will complete tasks when they connect to the cell tower. Thus, this algorithm predicts the probability of each worker connecting to different towers at least one time for the sensing period. We count the average number of connections by each worker $w_u$ at each cell tower $c_i$, which is denoted as $\lambda_{u,i}$. For example, we set the entire sensing period as one day. To estimate $\lambda_{u,i}$ for of a specific day, we count the average number of connections by $w_u$ at $c_i$ during each day in the historical mobility and connection records. Assuming that the connection sequence follows an inhomogeneous Poisson process [19,22,23], the probability of worker  $w_u$ to connect $h$ times to cell tower $c_i$ during a specific daycan be modeled as:
\begin{equation}
\varphi_{u,i}(h)=\lambda_{u,i}^{h}*e^{-\lambda_{u,i}}/h!
\end{equation}

Therefore, we can estimate the probability of worker $w_u$ connecting at least once during a day at $c_i$ as follows:
\begin{equation}
Pro_{u,i}=\sum_{h=1}^{\infty}\varphi_{u,i}(h)=1-e^{-\lambda_{u,i}}
\end{equation}

Thus we predict the probability of a candidate opportunistic worker  $w_u$ to complete task at $c_i$ as:
\begin{equation}
\alpha_i(w_u) = 1-e^{-\lambda_{u,i}}
\end{equation}

\subsubsection{Candidate solution generation}
In each iteration, HyTasker prefers to select the opportunistic workers who are not only capable of completing more tasks but also can complete tasks located in participatory-worker-sparse areas. Here, we introduce the concept of location entropy, which is proposed and applied in the social network community [31], to characterize the density of participatory workers in different locations. The intuition is that a location has higher entropy if many participatory workers visit that location with equal proportions. In contrast, a location will have lower entropy if the distribution of the visits to that location is restricted to only a few participatory workers. 

Inspired by this concept, we formally define the priority of each task based on its location entropy as follows:
\begin{equation}
Entropy(t_i)= -\sum_{pw\in PW_i}\frac{|Count_{pw,t_i}|}{|Count_{t_i}|}\times log\frac{|Count_{pw,t_i}|}{|Count_{t_i}|}
\end{equation}
\begin{equation}
Weight(t_i) = \frac{1/Entropy(t_i)}{\sum_{t\in T}(1/Entropy(t))}
\end{equation}

where $PW_j$ denotes the set of participatory workers visited the tower which $t_i$ belongs to, $Count_{t_i}$ denotes the times of the tower which $t_i$ belongs to was visited by $PW_i$, and $Count_{pw,t_i}$ denotes the times of worker $pw$ visited the tower which $t_i$ belonged to.

Then, the utility increase of adding one candidate opportunistic worker is calculated as follows:
\begin{equation}
Utility(OW_f\cup\{ow_j\}) - Utility(OW_f) = \sum_{t_i\in T}Weight(t_i)\times \varPhi(i,OW_f\cup\{ow_j\}) - \sum_{t_i\in T}Weight(t_i)\times \varPhi(i,OW_f)
\end{equation}

where $\varPhi(j,OW_f)$ will be illustrated with more details in section 4.2.3.

\subsubsection{Solution estimation and decision making}
At the end of each iteration, we record a snapshot, i.e., a subset of candidate opportunistic workers. Since we assume that each selected opportunistic worker will be given an equal reward, the total number of iterations will be $\lfloor\frac{B}{I_c}\rfloor$. In other words, we get $\lfloor\frac{B}{I_c}\rfloor$ possible solutions for the opportunistic worker selection. Then, we compare the optimality of them based on the following steps:  


First, we predict the probability of each task to be completed by a given subset of opportunistic workers. In Eq.(5), we have already obtained the probability of an opportunistic worker to complete each task. Thus, the probability that a task $t_i$ can be completed by a set of selected opportunistic workers $OW_f$ is defined as:
\begin{equation}
\varPhi(i,OW_f) = 1-\prod_{ow_i\in OW_f}(1-\alpha_i(ow_i))
\end{equation}

Second, we predict the optimal task assignments of the participatory workers by leveraging the maximum-flow-based algorithms [25,11]. In [25,11], the location of workers is known and all tasks are not completed. In contrast, in the offline worker selection phase of HyTasker, we only know the probability of predicted worker location and task completion status. Hence, we adopt multiple rounds of Monte-Carlo simulations to address this issue. Specifically, in each round of simulation, we construct the network of the maximum-flow based algorithm based on the probability of worker location and task completion status. The average number of completed tasks for multiple rounds of simulations is taken as the final result.


Third, we estimate the total number of completed tasks by both the opportunistic workers and the participatory workers. The subset of opportunistic workers with maximum estimated total number of completed tasks will be selected as the final output of the offline phase.

\subsection{Algorithm Complexity Analysis}
In this section, we analyze the time complexity of the proposed opportunistic worker selection algorithm. The inner-loop process of Algorithm~\ref{alg:OWS} needs to estimate the utility increase of all unselected opportunistic workers can make. The running time complexity of the inner-loop process of each iteration will be $O(|T|\times |OW|)$. After each iteration selects the best opportunistic worker, the task assignment of the participatory workers will consume $O(|PW|\times L\times (|PW|+|T|+C_{|T|}^{L}))$[11]. The outer-loop process will be run $\lfloor\frac{B}{I_c}\rfloor$ times, so the time complexity of Algorithm~\ref{alg:OWS} is $O(\lfloor\frac{B}{I_c}\rfloor\times (|T|\times |OW| + |PW|\times q\times (|PW|+|T|+C_{|T|}^{q})))$. 
